Images of the Ultra-High Energy Cosmic Rays from Point Sources

Our latest paper investigates the effects of UHECR propagation in a turbulent intergalactic magnetic field in the small-angle scattering regime, specifically focusing on the non-trivial caustic-like pattern that arises with strong deviation from isotropy. In this paper, we explore the effect of the observer's position on the measurement of source flux at a given distance. We examine three types of source locations, characterized by the density of cosmic rays from a given source at the observation point, which we call knots, filaments and voids. We also investigate the energy spectrum in these different cases and present simulated images of the source as it appears on the observer's telescope after propagation in the combination of intergalactic and Galactic magnetic fields. We show that hot spots in the UHECR data can arrive due to combined distortions of source images on the intergalactic and Galactic magnetic fields. Also the fact that flux of most nearby sources is diluted in the voids affects source population studies.

==> old.tex <==
%Accurately targeting a specific location can be challenging, particularly over long distances. Previous research, such as \cite{CRPropaLearns}, has explored methods for increasing the number of UHECR particles that hit a specific target, with the aim of improving the number of particles. This work provides a general idea for addressing the targeting problem in UHECR studies, which we build upon in our current research. 

% We use \texttt{CRbeam}\footnote{\url{https://github.com/okolo/mcray}}\cite{Kalashev_2023} code to simulate UHECR propagation. The original code allows to simulate the propagation of UHECRs, including interaction with CMB and turbulent magnetic field. In our modification, we added the possibility of emitting particles in the form of a jet with a given rotation angle and direction (including isotropically on a sphere), and also added the possibility of placing a spherical observer at an arbitrary point. It allows to obtain information about particles, including their momenta, which will be recorded by an observer located in a certain location, as in the previous study \cite{dolgikh2022causticlike}.

% \texttt{CRbeam} represents turbulent magnetic field with Kolmogorov's spectrum\cite{Giacalone_1999} as sum of hundreds waves with random direction in logarithmic scale by wavenumber (see \url{https://github.com/okolo/mcray/blob/main/src/lib/Deflection3D.cpp}). The small number of waves (40-50 waves for 20 Mpc) raise non-realistic artifacts, the big number of waves increase calculation time. We use 463 waves so the ratio of the wavenumbers of two adjacent waves is 1.01 in most cases. We keep the same random seed for magnetic field production for all simulations within the paper. \texttt{CRbeam} creates particles with random direction and simulates their propagation step by step throw magnetic field. This simulation uses \texttt{OpenMP} for multiprocessing acceleration.

% \input{targeting_mechanism}

% Optimization of the targeting mechanism was studied earlier in ref.\cite{CRPropaLearns}.  The authors used von Mises–Fisher distribution instead of simple cone jet and solve task for only one distance and energy. We reproduced this approach and modified it for our case.\

% At large distances, the problem of aiming at the observer arises. This is due both to a decrease in the angular size of the observer with distance and to the fact that statistically more often the observer finds himself in voids, where the cosmic ray flux is reduced.\

% Since we are examining the source images and flux excess/deficit at different distances or energies, we apply the following procedure for optimization of calculation time. First, we aim to observer from small distance $D_1$ where variation by magnetic field is negligible. After that we use the directions found on the preceding step at distance $D_i$ for aiming on distance $D_{i+1}>D_{i}$ ($D_{i+1}-D_{i}\sim 0.5-2 Mpc \lesssim r_g$ in our cases).\

% Another simulation parameter -- jet angle $\theta$ is chosen as previous minimal necessary jet angle multiplied by factor of $\sim 3$. We obtain minimal necessary jet angle from the analysis of particle directions in \texttt{CRbeam} output files. For the first run we choose $\theta_1\sim \frac{\pi}{2}$ or $\theta_1\gtrsim\arctan(\frac{R_{obs}}{D})$. If simulation has strong flux deficit, we recheck these results with $\theta\propto\sqrt{D\lambda_C}/E$ (see \cite{dolgikh2022causticlike}) and require the simulation to the HealPy map of the directions of departure of the hit particles was completely inside the emitted jet.

% To estimate the simulation acceleration factor, let's consider the figure. The flow can decrease by more than $\sim$100 times compared to the average at a distance of $\sim$20 Mpc, at this distance the observer occupies no more than $10^{-3}$ of the entire sphere. So, the probability of hitting an isotropically emitted particle is less than $10^{-5}$. Therefore, obtaining sufficient statistics would take a long time. Using the procedure explained above allows to direct particles into a cone with an angle of $\theta\sim 0.2$ radians and the geometric probability of hitting increases by about $2/(1-\cos(\theta)) \sim 100$ times. So, the figures~\ref{fig:images_all} have been simulated about 100 times faster than if the source was considered isotropic. 


% In other words, the simulation is restarted with a wide angle of the jet opening to check if particles are flying in from somewhere else. (Spoiler: I just got literally zero flux in observer even after a tens hours of watching the simulation, which confirmed the results of the previous simulation, but gave me confidence).




% \begin{figure}
%     \includegraphics[width=\linewidth]{Filament_D10Mpc_R100Kpc_bg.pdf}
%     \includegraphics[width=\linewidth]{Filament_D10Mpc_R100Kpc.pdf}
%     \caption{Example of source image in filament at $D=10$ Mpc, $B=1$ nG, $E=10^{19}$eV}
%     \label{fig:Filament1}
% \end{figure}
% \begin{figure}
%     \includegraphics[width=\linewidth]{Filament_D10Mpc_R100Kpc_E2_bg.pdf}
%     \includegraphics[width=\linewidth]{Filament_D10Mpc_R100Kpc_E2.pdf}
%     \caption{Example of source image in filament at $D=10$ Mpc, $B=1$ nG, $E=2*10^{19}$eV}
%     \label{fig:Filament2}
% \end{figure}

% \begin{figure}
%     \includegraphics[width=\linewidth]{Knot_D10Mpc_R100Kpc_bg.pdf}
%     \includegraphics[width=\linewidth]{Knot_D10Mpc_R100Kpc.pdf}
%     \caption{Example of source image in knot at $D=10$ Mpc, $B=1$ nG, $E=10^{19}$eV}
%     \label{fig:KnotImage}
% \end{figure}

% \begin{figure}
%     \includegraphics[width=\linewidth]{Void_D10Mpc_R200Kpc_bg.pdf}
%     \includegraphics[width=\linewidth]{Void_D10Mpc_R200Kpc.pdf}
%     \caption{Example of source image in void at $D=10$ Mpc, $B=1$ nG, $E=10^{19}$eV}
%     \label{fig:VoidImage1}
% \end{figure}




% Since we are examining the source images and flux excesses/deficits at different distances \textcolor{red}{and} energies, we apply the following procedure for optimization of calculation time. First, we aim to observer from small distance $D_\mathrm{1}$ where deflection by magnetic field is negligible \textcolor{blue}{and thus the aiming is trivial}. After that we use the directions found on the preceding step at distance $D_\mathrm{i}$ for \textcolor{blue}{optimizing} aiming parameters \textcolor{blue}{(a cone angle and a cone direction)} on distance $D_\mathrm{i+1}>D_\mathrm{i}$ ($D_\mathrm{i+1}-D_\mathrm{i}\sim 0.5-2$~Mpc~$\lesssim r_\mathrm{g}$ in our cases where $r_\mathrm{g}$ is gyroradius given by $r_\mathrm{g} =\frac{E}{\mid q\mid B}$).}

% \textcolor{blue}{The important} simulation parameter -- cone angle $\theta$ is chosen as previous minimal necessary cone angle multiplied by a constant factor. We have empirically seen that a value of $\sim 3$ for this factor allows to ensure that the most of the flux have not been missed. We obtain minimal necessary cone angle from the analysis of particle directions in \texttt{CRbeam} output files. For the first run we choose $\theta_1\sim \frac{\pi}{2}$ or $\theta_1\gtrsim\arctan(\frac{R_\mathrm{obs}}{D})$. If simulation has strong flux deficit, it is restarted with the wide angle of the cone $\theta\propto\sqrt{D\lambda_\mathrm{c}}/E$ (see \cite{dolgikh2022causticlike}) to ensure that all particles which may reach the observed are included into emitted cone.

% To estimate the simulation acceleration factor, let's consider the Fig.~\ref{fig:KnotDist}. The flux can decrease by more than $\sim$100 times compared to the average at a distance of $\sim$20 Mpc, at this distance the observer occupies no more than $10^{-3}$ of the entire \textcolor{blue}{set} of end particles coordinates. So, the probability of hitting an isotropically emitted particle is less than $10^{-5}$. Therefore, obtaining sufficient statistics would take a long time. Using the procedure explained above allows to direct particles into a cone with an angle of $\theta\sim 0.2$ radians and the geometric probability of hitting increases by about $2/(1-\cos(\theta)) \sim 100$ times. So, the Fig.~\ref{fig:images_all} have been simulated about 100 times faster than if the source was considered isotropic. 


%The observer may have a sufficiently large radius compared to the distance to source, which introduces some distortions in the apparent size of the source when naively constructing a HealPy\footnote{http://healpix.sf.net}\cite{2005ApJ...622..759G} map from the momentum of trapped particles. We remove this distortion by taking the projection of the particle's momentum on the Oz axis of our basis, which is parallels to the direction to the source. The second vector of the basis is chosen manually. We complete the basis by taking the cross product of first and second vectors.
